System Log Parsing: A Survey

Modern information and communication systems have become increasingly challenging to manage. The ubiquitous system logs contain plentiful information and are thus widely exploited as an alternative source for system management. As log files usually encompass large amounts of raw data, manually analyzing them is laborious and error-prone. Consequently, many research endeavors have been devoted to automatic log analysis. However, these works typically expect structured input and struggle with the heterogeneous nature of raw system logs. Log parsing closes this gap by converting the unstructured system logs to structured records. Many parsers were proposed during the last decades to accommodate various log analysis applications. However, due to the ample solution space and lack of systematic evaluation, it is not easy for practitioners to find ready-made solutions that fit their needs. This paper aims to provide a comprehensive survey on log parsing. We begin with an exhaustive taxonomy of existing log parsers. Then we empirically analyze the critical performance and operational features for 17 open-source solutions both quantitatively and qualitatively, and whenever applicable discuss the merits of alternative approaches. We also elaborate on future challenges and discuss the relevant research directions. We envision this survey as a helpful resource for system administrators and domain experts to choose the most desirable open-source solution or implement new ones based on application-specific requirements.

==> backup.tex <==
%!TEX root = main.tex

%\begin{table*}[h]
%\renewcommand{\arraystretch}{1}
%\caption{Prior work for quantitative performance evaluation and comparison works on existing log parsing solutions. For each work, we highlight the evaluated log parsers, the number of datasets along with their covered log entries, and the performance metrics, including accuracy (i.e., precision, recall, FM, PA, RI), efficiency, and memory footprint.}
%%%\vspace{-0.2cm}
%\label{tab:perf}
%\centering
%\footnotesize
%\begin{tabular}{|c||l||c|c||ccccc|c|c|c|}
%\hline
%\multirow{2}{*}{\bf Ref.} & \multirow{2}{*}{\bf Evaluated solutions} & \multirow{2}{*}{\bf Dataset} & \bf \#Entries & \multicolumn{5}{c|}{\bf Accuracy} & \multirow{2}{*}{\bf Efficiency} & \multirow{2}{*}{\bf Memory} \\ \cline{5-9}
%& & & ($\times 10^6$) &P &R &FM &PA & RI & &  \\ \hline \hline
%\cite{jiang2008abstracting} & AEL, SLCT& 201 & 1.73 & \checkmark & \checkmark &&&&& \\ \hline
%\cite{makanju2011lightweight}& IPLoM, SLCT, LogHound & 7 & 1.19 & \checkmark & \checkmark & \checkmark & & & \checkmark & \checkmark \\\hline
%\cite{gainaru2011event} & HELO, SLCT, LogHound, IPLoM & 5 & $\approx18.00$ & \checkmark & \checkmark& \checkmark& & & & \\ \hline
%\cite{tang2011logsig} & LogSig, IPLoM, StringMatch & 5 & 3.60 & & & \checkmark & & & & \\\hline
%\cite{mizutani2013incremental} & SHISO, IPLoM, SLCT & 2 & 0.60 & & & & & & \checkmark & \\ \hline
%\cite{hamooni2016logmine} & LogMine, HLAer & 5 & 10.04 & &&&& & \checkmark & \checkmark \\\hline
%\cite{he2016evaluation} & IPLoM, SLCT, LKE, LogSig & 5 & 16.44 & & & \checkmark &  & & \checkmark & \\ \hline
%\cite{he2017towards} & POP, SLCT, IPLoM, LKE, LogSig & 5 & 16.44 & && \checkmark& & & \checkmark & \\ \hline
%\cite{he2017drain} & Drain, IPLoM, Spell, SHISO, LKE& 5 & 16.44 &  & & \checkmark & & & \checkmark & \\ \hline
%\cite{guo2018event} &BSG, IPLoM, LogSig, Drain & 4 &16.12 & & & \checkmark & & & \checkmark & \\\hline
%\cite{zhao2018slop} & Slop, IPLoM, LogSig, Drain, Spell & 5 & 16.44 & \checkmark& \checkmark & \checkmark && & \checkmark & \\ \hline
%\cite{du2018spell} & Spell, Drain, IPLoM, LKE & 4 & 5.39 & \checkmark &\checkmark & \checkmark & \checkmark  & & \checkmark & \\ \hline
%\cite{vaarandi2015logcluster} & LogCluster, SLCT & 6 & - & &&& & & \checkmark & \\ \hline
%\cite{messaoudi2018search} & MoLFI, Drain, IPLoM& 6 & 16.44 & \checkmark& \checkmark & \checkmark & & & \checkmark & \\ \hline
%\cite{agrawal2019logan} & Logan, SHISO, Spell, Drain, IPLoM & 8 & 147.36 &&&& & & \checkmark & \\ \hline
%\cite{agrawal2019delog} & Delog, SHISO, Spell, Drain, IPLoM, Logan & 12 & 583.30 & &&& & & \checkmark & \\ \hline
%\cite{zhong2018flp} & FLP, Drain, Spell, IPLoM, LKE & 5 & 16.44 & & &\checkmark& & & \checkmark & \\ \hline
%\cite{yang2019online}& LogOHC, IPLoM, LogSig, Drain& 4 & 16.35 & \checkmark & \checkmark & \checkmark & & & \checkmark & \\ \hline
%\cite{tovarvnak2019normalization} & SLCT, IPLoM, LKE, LogSig, ENG& 5 & 16.44 & & & \checkmark & &  & &\\\hline
%\cite{zhang2019efficient} & CLF, MoLFI, Drain, IPLoM & 7 & 257.16 &  && \checkmark & & \checkmark & \checkmark & \\ \hline
%\cite{liu2019lopper} &Lopper, Drain, LogMine, LogSig, IPLoM & 8 & 16.62 & \checkmark & \checkmark & \checkmark & & & \checkmark & \\\hline
%\cite{wurzenberger2019aecid} & AECID-PG, SLCT, IPLoM, LKE, LogSig, Drain & 5 & 16.44 &  &  & \checkmark & & && \\\hline
%\multirow{2}{*}{\cite{zhu2019tools}} & SHISO, LogCluster, LenMa, LKE, SLCT, AEL, LFA& \multirow{2}{*}{16 }& \multirow{2}{*}{407.57} & & & & \multirow{2}{*}{\checkmark}  & & \multirow{2}{*}{\checkmark} & \\ 
%& LogSig, MoLFI, Spell, Drain, IPLoM, LogMine &&&&& && & & \\ 
%\hline
%\cite{huang2020paddy}& Paddy, LogMine, LenMa, Spell, Drain, MoLFI & 16 & 407.57 & & & & \checkmark & & \checkmark & \\\hline
%\multirow{2}{*}{\cite{studiawan2020automatic}} & Pylogabstract, IPLoM, LogSig & \multirow{2}{*}{5} & \multirow{2}{*}{0.14} & & & \multirow{2}{*}{\checkmark} & & & & \\ 
%& Drain, LogMine, Spell &&&&&&&&&\\ \hline
%\cite{liu2020web} & Drain, Spell, IPLoM & 1 & - & \checkmark & \checkmark & \checkmark & & && \\\hline
%\cite{chunyong2020log} & One-to-one, Drain, IPLoM, Spell & 3 & 16.13 & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & \\ \hline
%\cite{zhang2020efficient} & Craftsman, LogSig, IPLoM, LKE& 5 &16.44 &&&&  & \checkmark &  \checkmark& \checkmark \\\hline
%\cite{liu2020fastlogsim} & Spell, LogSig, SLCT, IPLOM, FastLogSim & 4 & 1.40 & &&& & & \checkmark & \\ \hline
%\cite{dai2020logram} & Logram, Drain, AEL, LenMa, Spell, IPLoM & 16 & 407.57 &  & && \checkmark & & \checkmark & \\ \hline
%%\multirow{2}{*}{\cite{xie2020confidence}} & AEL, Drain, LFA, MoLFI, SHISO, IPLoM, LenMa & \multirow{2}{*}{16}& \multirow{2}{*}{407.57} &&& &&&& \\ 
%%& LogCluster, LogMine, SLCT, LKE, LogSig, Spell & & & &&& && & \\\hline
%\cite{li2020swisslog} & SwissLog, Drain, Spell, AEL, IPLoM & 3 & 46.27 &  &  &  \checkmark & \checkmark & & & \\ \hline
%\multirow{2}{*}{\cite{nedelkoski2020self}} & NuLog,LenMa, Spell, Drain, BoA, LogSig, LKE, LFA & \multirow{2}{*}{10} &  \multirow{2}{*}{166.39} & & &  & \multirow{2}{*}{\checkmark} & & &\\ 
%& MoLFI, SLCT, AEL, LogCluster, SHISO, LogMine & & &&&& &&&\\ \hline
%\cite{coustie2020meting} & Drain, IPLoM, Spell, MoLFI, Logram, METING & 16 & 407.57 & & &  & \checkmark &  &&\\ \hline
%\cite{wen2020olmpt} & Drain, IPLoM, Spell, LogSig, SLCT, OLMPT & 5 & 16.44 & & & \checkmark &  & & \checkmark &\\ \hline
%\cite{xiao2020lpv} & LPV, Drain, Spell & 3 & 16.35 & \checkmark & \checkmark & \checkmark& \checkmark & &  \checkmark &\\ \hline
%\cite{wang2021ltmatch} & LenMa, Spell, AEL, IPLoM, Drain, LTmatch & 16 & 407.57 & & & & \checkmark & & \checkmark &\\ \hline
%\cite{chu2021prefix} & FT-tree, Drain, Spell, IPLoM, AEL, Prefix-Graph & 10 & 17.99 & & & & & & \checkmark &\\ \hline
%\cite{aussel2018improving} & NLP-LP, Drain, POP, SLCT, LogSig, IPLoM & 1 & 11.18 & \checkmark & \checkmark & \checkmark &&&& \\ \hline
%\cite{zhang2017syslog} & FT-tree, STE, LogSimilarity, Signature Tree & 4 & 0.002 &&&&& \checkmark & \checkmark &\\ \hline
%\cite{chu2021prefix} & FT-tree, Drain, Spell, Spell, Log2Vec, template2Vec & 4 & 159.41 & & & \checkmark &&& &\\ \hline
%\cite{duan2021oilog} & OILog, LogSig, STE, LogSimilarity, Spell & 4 & 44.81 & & & \checkmark & & & \checkmark &\\ \hline
%%\cite{meng2019loganomaly} &&&&&&&&&&\\ \hline
%%&&&&&&&&&&\\ \hline
%\end{tabular}
%\end{table*}

\section{Performance features}\label{sec:perf}
Although the large collection of log parsers, correctly choosing and configuring the most suitable solutions is still non-trivial. As existing log parsers are implemented with different algorithms, they have divergent performance features and configuration complexities. Misconfigured parsers can lead to severe performance degradation for the ensuing log mining and analytic tasks. As a result, we devote this section to empirically analyzing the quantitative (Sec. \ref{sec:perf-char}) and qualitative (Sec. \ref{sec:features}) features of the existing solutions.

\subsection{Quantitative features}\label{sec:perf-char}
We review two key quantitative features in this work, namely the {\it parsing accuracy} and {\it execution time} of the existing solutions in Sec. \ref{sec:accuracy} and Sec.~\ref{sec:efficiency}.
Due to the huge number of solutions and absence of source code for a subset of them, quantitatively comparing the performance of all the existing solutions is impractical. Therefore, we opt to conduct our empirical analysis in a hybrid fashion combining both the available results in the literature and the quantitative evaluation on the open-source log parsers.


\subsubsection{Parsing accuracy}\label{sec:accuracy}
Conventionally, there are three classic metrics to measure the effectiveness of information retrieval, i.e., {\bf Precision, Recall}, and {\bf F-Measure (FM)}. The precision is the ratio of correctly parsed log pairs over the total pairs generated by a log parser. By definition, recall is the ratio of correctly parsed log pairs over the actual total log pairs. 
Precision and recall are calculated as follows:
\begin{equation}
Precision = \frac{TP}{TP+FP}
\end{equation}
\begin{equation}
Recall = \frac{TP}{TP+FN}
\end{equation}

In the context of log parsing, given $N$ raw input log entries (i.e., $\frac{N(N-1)}{2}$ message pairs), a true positive (TP) decision correctly identifies two log messages of the same type, a false positive (FP) decision arbitrates two log messages of different types to the same group, while a false negative (FN) decision parses two log messages of the same type to different groups. Precision and recall can reflect the effectiveness of existing solutions. In essence, under-parsing can result in more false positives and degrade precision, while over-parsing can lead to more false negatives and hurt recall. F-Measure (or F-score) is purposed to balance these two metrics and it is calculated as follows: 
\begin{equation}
FM= \frac{(\beta^2+1)\cdot Precision \cdot Recall}{\beta^2 \cdot Precision + Recall}
\end{equation}
where $\beta$ is conventionally set to 1. 
Although FM can reflect log parsing accuracy, it only accounts for the correctly parsed log pairs, which is insufficient for log parsing. According to the definition of FM, two log messages of the same type are still considered a correct pair even if they are parsed into the a group different from the rest of the same-typed log messages. Instead of FM, Du et al.~\cite{du2018spell} proposed the {\bf Parsing Accuracy (PA)} to account for the ratio of correctly parsed log messages over the total number of log messages. PA is formally calculated as: 
\begin{equation}\label{eq1}
PA = \frac{\# Correct{\_}Messages}{\# Total{\_}Messages}
\end{equation}
Note that, for the numerator in equation~\ref{eq1}, log messages belonging to the same event type are considered correctly parsed if and only if all of them are parsed to the same group; otherwise, none of these messages is regarded as correct. Therefore, PA is more strict than FM and is more suitable to evaluate the log parsing accuracy. We thus choose PA as the accuracy metric for our experiments. 

\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/f1}
\caption{The average F-Measure for some log parsers extracted from the literatures.}
\label{fig:f1}
\end{center}
\end{figure}

\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/pa}
\caption{The Parsing Accuracy distribution for some log parsers over heterogeneous logs.}
\label{fig:pa}
\end{center}
\end{figure}

According to our literature review, approximately 50 papers evaluated the performance of different log parsers. These works used a variety of public/proprietary logs as datasets to compare the selected log parsers in terms of standard or customized performance metrics. Most of these related works used FM and PA to characterize the accuracy of existing log parsers\footnote{Note that some related works evaluated log parsing accuracy with {\em Rand Index (RI)}, which is calculated as: $\frac{TP + TN}{TP + FP + FN + TN}$. We omit RI in our study since it is not as commonly employed as the FM and PA. Please refer to \cite{zhang2019efficient,chunyong2020log,zhang2020efficient,tao2021logstamp,zhang2017syslog} for RI-related evaluation.}.
Therefore, we first capitalize on the numerical results in the literature to empirically understand the achievable accuracy for existing solutions. We thus collect all the numerical results and calculate the average FM and PA of existing log parsers in Fig.~\ref{fig:f1} and Fig.~\ref{fig:pa}. Although the comparisons are biased because the evaluation datasets and runtime configurations were not exactly the same for all the log parsers, they can still help us develop a general idea. 
As we can observe, most of the log parsers can achieve $\geq 80\%$ FM and $\geq 57\%$ of them can even reach $\geq 90\%$. 

Despite PA is more strict than FM (as explained before), most of the parsers can still attain $\geq 60\%$ PA, which is reasonable given the heterogeneity of the validation logs. With proper parameter tuning and preprocessing (which will be discussed later), their accuracies are expected to improve. 
In general, state-of-the-art solutions such as SLCT, LogMine, LogSig, LKE generally perform worse than newly proposed ones. This is partially because the former are more widely evaluated than the latter. Although some newly proposed solutions, such as FastLogSim, ENG, FLP, and One-to-One, can achieve near $100\%$ FM, their high accuracies can be biased since they were only tested with the limited datasets. 

\begin{table}[!tb]
\caption{Main characteristics of LogHub's 16 datasets}
\vspace{-0.3cm}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\bf Dataset & \bf Log messages & \bf Message length & \bf \#Templates (2k) \\ \hline
BGL & 4,747,963 & 10 $\sim$ 102 & 376 \\\hline
HDFS & 11,175,629 & 8 $\sim$ 29 & 29 \\\hline
HPC & 433,490 & 6 $\sim$104 & 105 \\\hline
Proxifier & 10,108 & 10 $\sim$ 27 & 8 \\\hline
Zookeeper & 74,380 & 8 $\sim$ 27 & 80 \\\hline
Linux & 25,567 && \\\hline
HealthApp & 25,3395 && \\\hline
Apache & 56,481&& \\\hline
Spark & 33,236,604 && \\\hline
Hadoop & 394,308 && \\\hline
OpenSSH & 655,146 && \\\hline
OpenStack & 207,820 && \\\hline
Windows& 114,608,388 && \\\hline
Android & 1,555,005 && \\\hline
Thunderbird & 211,212,192 && \\\hline
Mac & 117,283 && \\\hline 
\end{tabular}
\end{center}
\label{tab:dataset}
\vspace{-0.5cm}
\end{table}%

\begin{figure*}[!tb]
\begin{center}
\includegraphics[width=\textwidth]{figures/accuracy_dist}
\caption{The Parsing Accuracy distribution for some log parsers over heterogeneous logs.}
\label{fig:accuracy_dist}
\end{center}
\end{figure*}

Albeit the optimistic results, some solutions were only evaluated on a few datasets, and it is unclear if they can sustain similar effectiveness on other system logs. Therefore, we decide to complement existing works by thoroughly evaluating the open-source log parsers. We measure the PA of 17 open-source log parsers, namely LogSig, LKE, SLCT, LFA, MoLFI, SHISO, LogCluster, LogMine, AEL, Spell, LenMa, IPLoM, Drain, Logram, Paddy, NuLog, and SwissLog. The source code of the first 13 solutions are provided by the LogPAI team~\cite{zhu2019tools,he2016evaluation}. Note that other projects such as amuLog~\cite{kobayashi2020amulog} and LogParse~\cite{meng2020logparse} also provided implementations for some of these log parsers (e.g., Drain, LogSig, etc.). We decide to stick to the LogPAI's solutions, because they have already been widely employed by both industry and academia. The last 4 solutions were also implemented following the interface of LogPAI. 
Note that we are aware of other open-source solutions (e.g., FLP, Pylogabstract, Log2Vec, and LogDTL), we exclude them from our evaluation due to lack of information or limited customizability. Integrating them is left for future work. 

We reuse the 16 datasets of LogHub~\cite{he2020loghub} to validate the PA of these solutions. The main characteristics of these datasets are shown in Table~\ref{tab:dataset}. Each dataset has 2k log entries randomly sampled from the original system logs. The ground-truth event types and log templates have already been manually extracted for validation. These datasets cover a variety of ICT systems including distributed computing, operating systems, supercomputers, and software apps, and performance evaluations across this dataset ensemble can fairly validate the effectiveness of a log parser over heterogeneous logs~\cite{he2020loghub}. Following the approaches by Zhu et al.~\cite{zhu2019tools}, We measure the PAs of the 17 log parsers on all datasets. To ensure the optimality of the obtained results, we extensively tune the parameters of each log parser. 
For non-deterministic solutions like LKE, MoLFI, and NuLog, we repeat the experiments 10 times to obtain the averages. Note that NuLog was only evaluated on 10 of the 16 datasets, because the authors did not provide the related regex rules and parameters. We will discuss preprocessing and parameter tuning at length in the next section.

We plot the distribution of PA all the log parsers under test in Fig.~\ref{fig:accuracy_dist}, ranked from left to right in ascending order of the median. In general, no solution can consistently prevail in all the test scenarios. Based on our observation, the accuracy of each log parser varies on different datasets. This is quite intuitive since each solution was designed to explore specific features of system logs. If the input logs deviate from the expected formats, the accuracy is expected to decrease. 
For relatively simple datasets like Apache, almost all the solutions can achieve $100\%$ PA (except LogSig, which presents the lowest overall accuracy, as it is challenging to specify the cluster numbers beforehand). As the log complexities increase, the effectiveness of these solutions begin to diverge. As we observe, the accuracy of IPLoM degrades on system logs with highly varied message lengths, SLCT and LFA cannot identify infrequent patterns below the threshold. The most extreme case is MoLFI, which achieves only $0.8\%$ PA on the Proxifier dataset since it has difficulty distinguishing event types with highly similar formats. Actually, MoLFI does achieve $74\%$ FM on the same dataset, which means it under-parses the identified messages, leading to extremely low PA. This case also validates the necessity of using PA as accuracy metric over FM.
In fact, even the overall performant solutions still possess deficiencies on specific logs, e.g., Drain performs poorly on datasets with a lot of leading variable tokens (e.g., Mac). Based on the obtained result, NuLog and SwissLog achieve the best overall accuracy. NuLog has the highest overall PA (mean $94.3\%$, median $98.9\%$) and stability, which proves the adaptability of neural networks for log parsing. Other heuristic solutions such as Drain, and AEL also show promising results. In general, heuristic solutions outperform solutions based on clustering and frequent pattern mining. 

%Most of the prior works evaluated the log parsing accuracy based on these metrics. For instance,
%Jiang et al.~\cite{jiang2008abstracting} evaluated the precision and recall of SLCT and AEL on 201 log files collected from an enterprise application %, including 100 randomly sampled small log files (each with 100 entries), 100 randomly sampled medium-sized log files (each with $10k$ entries), and a large log file ($723k$ entries). 
%AEL consistently outperformed SLCT in all experiments, as the latter can only identify log templates whose occurrence is beyond the threshold.
%In \cite{makanju2011lightweight}, the precision, recall, and F-Measure of SLCT, LogHound, and IPLoM were evaluated on 7 system logs. %, including the public HPC dataset, 4 private datasets collected from faculty networks, and 2 from ISP servers. 
%IPLoM achieved the highest overall accuracy. SLCT slightly outperformed LogHound, as the latter cannot detect log messages with trailing variable tokens.
%Tang et al.~\cite{tang2011logsig} compared the FM of LogSig, IPLoM, and StringMatch on 5 datasets collected from real systems. LogSig achieved the best overall accuracy while IPLoM and StringMatch struggled on log events with varied message lengths. However, LogSig always required the number of clusters as an input parameter, which is challenging to decide beforehand.
%Mizutani et al.~\cite{mizutani2013incremental} leveraged a security system log ($\approx12k$ messages) to compare the parsing accuracy of SHISO, SLCT, and IPLoM. SHISO had the highest accuracy according to their results. 
%In \cite{vaarandi2015logcluster}, SLCT and LogCluster were compared on 6 datasets collected from a national institute. For the identified clusters, LogCluster did not have the overfitting problem faced by SLCT. 

%\begin{table*}[!tb]
%\caption{Time complexity of the solutions under evaluation}
%\tiny
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
%& LogSig & Logram & LFA & MoLFI & LogCluster & SHISO & SLCT & LogMine & LKE & Spell & IPLoM & Paddy & LenMa & Drain & AEL & SwissLog & NuLog \\ \hline
%Complexity &&&&&&&&&&&&&&&&&\\ \hline
%\end{tabular}
%\end{center}
%\label{default}
%\end{table*}%

\begin{figure*}
    \centering
    \setkeys{Gin}{width=0.33\linewidth}
\subfloat[Apache]{\includegraphics{figures/efficiency_Apache}}% 1
\hfill
\subfloat[OpenSSH]{\includegraphics{figures/efficiency_OpenSSH}}% 2
\hfill
\subfloat[OpenStack]{\includegraphics{figures/efficiency_OpenStack}}% 3
\hfill
\subfloat[BGL]{\includegraphics{figures/efficiency_BGL}}% 4
\hfill
\subfloat[Zookeeper]{\includegraphics{figures/efficiency_Zookeeper}}% 5
\hfill
\subfloat[Linux]{\includegraphics{figures/efficiency_Linux}}% 6
\hfill
\subfloat[HDFS]{\includegraphics{figures/efficiency_HDFS}}% 7
\hfill
\subfloat[Hadoop]{\includegraphics{figures/efficiency_Hadoop}}% 8
\hfill
\subfloat[Spark]{\includegraphics{figures/efficiency_Spark}}% 9
\hfill
\subfloat[HPC]{\includegraphics{figures/efficiency_HPC}}% 10
\hfill
\subfloat[Proxifier]{\includegraphics{figures/efficiency_Proxifier}}% 11
\hfill
\subfloat[HealthApp]{\includegraphics{figures/efficiency_HealthApp}}% 12
\caption{The log parsing time of 16 open-source log parsers on sample datasets with different number of log entries.}
\label{fig:efficiency-samples}
\end{figure*}

%With the availability of more public log datasets, later research managed to deliver reproducible results. Some of the most commonly adopted datasets are listed in Table \ref{tab:dataset}. 
%These are among the 16 log datasets published by LogHub~\cite{loghub}.
%These datasets contain a divergent number of messages and event types. For instance, HDFS has 524$\times$ more messages than Proxifier but only twice the number of event types. The Linux dataset inversely has 54 times more event types than Proxifier but with almost the same number of messages. %Large datasets have several orders of magnitude more messages and event types than most of the others. 
%These datasets also have a different number of words, constant tokens, and variable tokens~\cite{wang2021ltmatch}. The heterogeneity of these datasets allows them to be used to assess the performance of existing log parsers. 
%
%To avoid the overly long execution time of some solutions on large datasets, these works randomly extract small samples (e.g., 2k log messages) from these datasets for performance evaluation. 
%For instance, 
%He et al.~\cite{he2016evaluation,he2017towards} used the five datasets to compare SLCT, IPLoM, LKE, POP, and LogSig. 
%IPLoM achieved the best overall accuracy on raw logs. But after proper preprocessing to remove numerical parameters, LogSig outperformed IPLoM and SLCT. LKE had the worst accuracy due to its aggressive clustering. 
%POP had the best overall parsing accuracy thanks to its fine-grained partitioning that avoids over-fitting.
%He et al.~\cite{he2017drain} compared Drain, IPLoM, Spell, SHISO, and LKE. Drain had the highest overall FM because it simultaneously considered both message length and leading tokens to build clusters, effectively avoiding over-partitioning on most datasets. IPLoM and Spell had very close accuracies to Drain. SHISO employed character-wised similarity to guide the search process, which can lead to inaccuracy. 
%Guo et al.~\cite{guo2018event} compared BSG, IPLoM, LogSig, and Drain on the 2K samples of 4 datasets, including BGL and HDFS. BSG achieved the highest FM. LogSig presented the lowest accuracy due to the impact of its random initialization. Drain performed poorly on log messages with leading tokens as variables. 
%Messaoudi et al.~\cite{messaoudi2018search} compared MoLFI, Drain, and IPLoM. MoLFI outperformed Drain by $13-36\%$ and IPLoM by $20-81\%$ as its customized NSGA-II genetic algorithm can significantly improve both precision and recall after enough generations. 
%Studiawan et al.~\cite{studiawan2020automatic} compared their proposed algorithm with IPLoM, LogSig, Drain, LogMine, and Spell on 5 public forensic datasets. Their method achieved the highest FM because they employed the weighted Hamming similarity, which considers the token order and prioritizes the leading tokens. 

%Besides the commonly used metrics, some works defined a more strict Message Level Parsing Accuracy (PA), the ratio of correctly parsed messages over the total number of parsed messages. A log message is deemed as rightly parsed if and only if its constant and variable parts perfectly match the ground truth. Partially matched 
%Zhu et al.~\cite{zhu2019tools} extensively compared 13 state-of-the-art log parsers using the 16 public datasets from LogHub~\cite{loghub} with minimal preprocessing. Drain achieved the highest PA on 9 datasets. IPLoM, AEL, and Spell attained $\geq 90\%$ accuracy on 6 datasets. LKE and LogSig had the lowest accuracy. 
%Li et al.~\cite{li2020swisslog} compared the PA of SwissLog with the same log parsers and datasets. SwissLog outperformed these state-of-the-art solutions with an average PA of $96\%$ and achieved $100\%$ accuracy on 5 datasets. The authors attributed the edge of SwissLog to the benefits of dictionary-based parsing. 
%Huang et al.~\cite{huang2020paddy} compared the PA of LogCluster, LogMine, LenMa, Spell, Drain, MoLFI, and Paddy on the same datasets. Paddy had the highest average accuracy ($89\%$) and negligible variance because it employed a dynamic dictionary for easy indexing and combined Jaccard similarity and message length to rank the extracted templates. 
%Dai et al. \cite{dai2020logram} compared the Logram, Drain, AEL, LenMa, Spell, and IPLoM on the same datasets. Logram achieved the best accuracy (with over $90\%$ PA on 12 datasets) thanks to its token-based parsing. 
%Coustie et al.~\cite{coustie2020meting} compared the PA of Drain, IPLoM, Spell, MoLFI, Logram, METING using the 16 datasets of LogHub. METING achieved the highest average accuracy ($90.5\%$) as its dendrogram representation and n-gram splitting can effectively deal with the various message formats. Drain had the second-best accuracy, but it could not identify templates with leading variable tokens. IPLoM has trouble with logs of different lengths. Spell cannot distinguish two event types with highly similar LCS. 
%Du et al.~\cite{du2018spell} compared the performance of an upgraded Spell to Drain, IPLoM, and LKE using 4 datasets, including the BGL, HPC, and two datasets from a cloud testbed. The most recent Spell implementation achieved the highest accuracy because its split and merge operations can effectively readjust the parsing results to avoid over- and under-parsing.
%In \cite{zhang2020efficient}, Craftsman, LogSig, IPLoM, and LKE were compared in terms of Rand Indexes (RI), which is computed as $\frac{TP + TN}{TP + FP + FN + TN}$. Craftsman and IPLoM achieved the best rand indexes ($96.25\%$ and $93.86\%$) thanks to their effective heuristic rules that adapt to various formats.
%Chu et al.~\cite{chu2021prefix} evaluated the RI of FT-tree, Drain, Spell, IPLoM, AEL, and Prefix-Graph. Prefix-Graph achieved the highest accuracy of 7 of the 10 datasets. 
%
%Some works also studied the accuracy of existing log parsers, but they either did not discuss their experimental results at length or conducted the evaluation using limited datasets. We report their findings here for references: 
%Gainaru et al.~\cite{gainaru2011event} compared the precision, recall, and FM of HELO, SLCT, LogHound, and IPLoM on 5 log datasets of supercomputers. HELO achieved optimal accuracy in all the experiments.
%Zhao et al.~\cite{zhao2018slop} evaluated the accuracy of Slop, IPLoM, Drain, and Spell. Slop achieved the best precision, accuracy, and FM, while Spell and Drain severely suffered from overfitting due to improper parameter settings.
%Zhong et al.~\cite{zhong2018flp} evaluated the performance of FLP, Drain, Spell, IPLoM, and LKE. FLP achieved optimal accuracy. %, but the authors did not give detailed explanations of the experimental results.
%Tovarvnak et al. \cite{tovarvnak2019normalization} measured the FM of SLCT, IPLoM, LKE, LogSig, and ENG. ENG had the highest FM.
%Agrawal et al.~\cite{agrawal2019logan, agrawal2019delog} evaluated the parsing accuracy of Logan, SHISO, Spell, Drain, Delog, and IPLoM using a customized metric and claimed that Logan and Delog delivered the best parsing quality. 
%Zhang et al.~\cite{zhang2019efficient} compared the FM and PA of MoLFI, Drain, IPLoM, and CLF. All the solutions achieved similar FM, but CLF had sightly higher PA than others. 
%Liu et al.~\cite{liu2020fastlogsim} compared Spell, Drain, IPLOM, and FastLogSim on the HDFS dataset. FastLogSim, Spell, and Drain achieved comparable results.
%Yang et al.~\cite{yang2019online} compared IPLoM, Drain, Spell, and LogOHC. LogOHC achieved slightly better precision, recall, and FM. 
%Zhang et al.~\cite{chunyong2020log} compared IPLoM, Drain, Spell, and One-to-One using the BGL, OpenStack, and HDFS datasets. One-to-One achieved the best accuracy. 
%Liu et al.~\cite{liu2020web} compared their proposed log parser with Spell, Drain, and IPLoM on a Chinese weblog. Their solution outperformed the others by the keyword-based parsing can better process Chinese logs. 
%Liu et al.~\cite{liu2019lopper} compared Lopper, Drain, LogMine, IPLoM, and LogSig. Lopper achieved the overall highest precision, recall, and FM. 
%Wurzenberger et al.~\cite{wurzenberger2019aecid} compared AECID-PG, SLCT, IPLoM, LKE, LogSig, and Drain. AECID-PG achieved the highest overall FM (i.e., $94\%$) in their experiments. 
%Nedelkoski et al.~\cite{nedelkoski2020self} compared NuLog with state-of-the-art solutions. Their results showed that NuLog outperformed other solutions by $4-13\%$ in terms of PA. 
%Wen et al.~\cite{wen2020olmpt} evaluated the FM of Drain, IPLoM, Spell, LogSig, SLCT, and OLMPT. OLMPT achieved at least $89\%$ FM on all the 5 datasets of Table~\ref{tab:dataset}. 
%Xiao et al.~\cite{xiao2020lpv} evaluated the precision, recall, FM, and PA of Drain, Spell, and LPV. LPV achieved the highest overall accuracy. 
%Wang et al.~\cite{wang2021ltmatch} compared the PA of LenMa, Spell, AEL, IPLoM, Drain, and LTmatch on the 16 datasets of LogHub. LTmatch achieved the highest average accuracy ($88.85\%$)

\subsubsection{Parsing time}\label{sec:efficiency}
Besides accuracy, parsing time is another critical performance metric, especially for real-time log analysis tasks. In this section, we characterize the execution time of 16 open-source log parsers.  To ensure fair comparison, all the experiments are conducted on a commodity server equipped with Intel Xeon CPU E5-2670 @ 2.3GHz (48 cores across two NUMA nodes) and 64GB RAM. The each experiment is purposely assigned to execute on isolated CPU cores to reduce system-level interference. Since the log parsers under test are all implemented as single-thread applications, we assign one CPU core to each solution for latency test. To ensure fair comparison, we use the online version of Logram (without the Spark acceleration). We also exclude NuLog from this evaluation as its neural network training is much slower than other solutions, even with GPU acceleration. 
We select 12 datasets from LogHub, i.e., the first 12 datasets in Table~\ref{tab:dataset}, and randomly sample log entries to compose the validation datasets. The sample sizes include 4k, 10k, 16k, 20k, 30k, 40k, 50k, 60k, 70k, 80k, 90k, and 100k. Similar to prior works, the default parameters and preprocessing rules remain the same for all solutions.


We measure the execution time for each solution on all the datasets and illustrate the results in Fig.~\ref{fig:efficiency-samples}. 
As some log parsers, especially LKE, require excessively long execution time to parse large log samples, we skip the experiments at some point to save time, yet the general trend still holds. As we can observe, the execution time for most of the solutions can approximately scale linearly as the sample size grows. 
The heuristic solutions achieve lower overall execution time than other solutions. In particular, IPLoM, SwissLog, AEL, Spell, and Logram consistently achieve low execution time, and they can finish parsing 100k log files in around 10 seconds. These heuristic solutions use simple data structures and control logics that can greatly reduce the parsing time. The execution time of offline clustering-based solutions, i.e., LKE, LogMine, and LogSig, also scale linearly with sample size, but they take considerably longer time to finish. LKE presents the highest parsing time due to its $O(n^2)$ time complexity, making it incapable of processing large datasets in a reasonable time. LogMine is also slow mainly because of its huge message merging overhead. LogSig performs slightly better, but its clustering method is still slow to converge, and its execution time also depends on the starting point.

The execution time of other solutions are quite divergent across different datasets even if the total number of log entries are the same, which means there are other factors that can also impact their execution time. 
For instance, 
LenMa parses logs slower than other heuristic solutions as its time complexity is related to message length, so it is generally less performant on datasets with many long messages (e.g., HPC, BGL).  
MoLFI has comparable result to LenMa on most datasets, but its execution time increases by a large margin on the distributed systems datasets (e.g., Hadoop, HDFS, Spark, and OpenStack) with more diversified log formats.
SLCT is the only solution that does not scale linearly on most of the datasets. This is because SLCT relies on the frequent tokens to match the log messages for pattern mining. As the sample size increases, so is frequent words set, which consequently increases the computation overhead of SLCT. This phenomenon is particularly obvious on complex datasets that contain large vocabularies, which explains the SLCT's sudden jump on complex datasets such as Spark, Hadoop, and HPC. Note that there are also unexpected behaviors presented by some solutions on specific datasets (e.g., Spell's fluctuation on $\geq 40k$ HealthApp datasets). We just focus on the more general trends in this paper and the more peculiar results calls for further case studies.

%For instance, 
%Makanju et al.~\cite{makanju2011lightweight} reported that SLCT had a similar execution time as LogHound and IPLoM on small datasets ($\leq 24k$ messages) but outperformed them on larger ones. The authors also explained the limitations of IPLoM and gave suggestions to improve efficiency. 
%Tang et al.~\cite{tang2011logsig} reported IPLoM achieved better efficiency than LogSig and StringMatch, thanks to its more straightforward processing logic. 
%Mizutani et al.~\cite{mizutani2013incremental} measured the parsing time of SHISO, IPLoM, and SLCT. Their results indicated SHISO was the most efficient solution. %In particular, SLCT outperformed IPLoM by a large margin, which was consistent with the results in \cite{jiang2008abstracting}. 
%Vaarandi et al.~\cite{vaarandi2015logcluster} evaluated the efficiency of SLCT and LogCluster and reported that SLCT was 1.28–1.62 times faster. 
%Hamooni et al.~\cite{hamooni2016logmine} compared HLAer and LogMine. According to their results, LogMine was up to 500 times faster than HLAer since it can process logs in a single pass using a more efficient pattern recognition scheme. 
%He et al.~\cite{he2016evaluation} evaluated the efficiency of SLCT, IPLoM, LogSig, and LKE. The parsing time of SLCT and IPLoM can scale linearly with the sample size. SLCT slightly outperformed IPLoM because of its relatively simpler processing logic. LKE presented the worst efficiency due to its $O(n^2)$ time complexity, making it incapable of processing large datasets, such as BGL and HDFS, in a reasonable time. LogSig had a better efficiency than LKE but still struggled with large data samples.
%He et al. \cite{he2017drain} compared the execution time of Drain, IPLoM, Spell, SHISO, and LKE. Drain achieved the lowest execution time for all the experiments. 
%According to \cite{guo2018event}, BSG, IPLoM, and Drain incurred similar processing time as they feature the same computation complexity ($O(N)$). LogSig had the worst efficiency as its clustering method is slow to converge and highly reliant on the actual starting point.
%
%Zhao et al.~\cite{zhao2018slop} compared the parsing time of Slop, IPLoM, LogSig, Drain, and Spell on samples of different sizes. LogSig required the longest parsing time due to the grouping overhead. Slop incurred the least parsing time on almost all datasets as it required fewer comparisons in each partition. 
%Zhong et al. \cite{zhong2018flp} evaluated the efficiency of FLP, Drain, and IPLoM. FLP had the shortest parsing time thanks to its $O(\log_2 N)$ complexity. 
%Messaoudi et al.~\cite{messaoudi2018search} compared MoLFI, Drain, and IPLoM. Drain is generally the most efficient solution for small log files, while IPLoM achieved the best efficiency with more than 100K messages. MoLFI was the slowest because its genetic algorithm requires many rounds to generate acceptably accurate Pareto frontiers.
%Dai et al. \cite{dai2020logram} evaluated the efficiency of Logram, Drain, AEL, LenMa, Spell, and IPLoM on samples from 5 datasets of LogHub. %The efficiency is compared by measuring the parsing time on randomly extracting data chunks of 300KB, 1MB, 10MB, 100MB, 500MB, and 1GB from 5 datasets.
%The sample size varies from 300KB to 1GB. Their results show that Logram outperformed others by 1.8 to 5.1 times.
%Huang et al.~\cite{huang2020paddy} compared the efficiency of Paddy with MoLFI, LenMa and Drain using samples of different sizes on two datasets of LogHub. Drain incurred the least processing time and slightly outperformed Paddy. LenMa and MoLFI failed to parse 1G of BGL logs.
%Agrawal et al.~\cite{agrawal2019logan,agrawal2019delog} evaluated the efficiency of Logan, SHISO, Spell, Drain, Delog, and IPLoM. Logan and Delog had the least parsing time. %However, the authors did not give any insights into the results. 
%Zhang et al.~\cite{zhang2020efficient} measured the parsing time of Craftsman, IPLoM, LogSig and LKE on the BGL dataset. Craftsman took only 5 seconds to parse the data thanks to its efficient heuristic design. In comparison, IPLoM, LogSig, and LKE took 37 minutes, 19.7 hours, and 5.4 days, respectively. 
%Liu et al.~\cite{liu2019lopper} compared the efficiency of Lopper, Drain, LogMine, IPLoM, and LogSig. Lopper, IPLoM, and Drain had the best efficiency as they all have $O(n)$ time complexity. LogMine incurred $O(l_1 \times l_2)$ time to merge two log records of length $l_1$ and $l_2$. LogSig had the worst efficiency due to its $O(n^2)$ complexity. 
%%The efficiency of Spell, LogSig, SLCT, IPLOM, and FastLogSim were also compared in \cite{liu2020fastlogsim}. FastLogSim achieved the highest efficiency on the HDFS dataset. 
%Zhu et al.~\cite{zhu2019tools} measured the parsing time of MoLFI, Spell, LenMa, IPLoM, AEL and Drain on the HDFS, BGL, and Android datasets. Drain and IPLoM had the best efficiency because of their linear time complexity. AEL also performed well on all HDFS and Android but incurred huge time on BGL over the 500MB sample size due to many generated bins. Other parsers failed to scale with the volume of input logs. As reported by the authors, LenMa and MoLFI could not even finish parsing 1GB BGL and Android in 6 hours.
%Wen et al.~\cite{wen2020olmpt} analyzed the efficiency of Drain, IPLoM, Spell, LogSig, SLCT, and OLMPT. SLCT had the best efficiency on small datasets, but its advantage faded on large datasets due to the overhead of passing the input dataset multiple times. LogSig had the lowest efficiency, and its parsing time does not grow linearly with the input data size. 
%Chu et al.~\cite{chu2021prefix} measured the parsing time of FT-tree, Drain, Spell, IPLoM, AEL, and Prefix-Graph on the HDFS and BGL datasets. AEL had the best efficiency and required an average of 24 s to parse 1 million logs and outperformed Prefix-Grap (57 s), FT-tree (80 s), Drain (91 s), IPLoM (93 s), and Spell (121 s). 
%Du et al.~\cite{du2018spell} compared the efficiency of an upgraded version of Spell with Drain, IPLoM, and LKE. Spell adopted several optimization methods in its pre-filtering step to amortize the entry lookup cost. It managed to run faster than IPLoM and LKE and was close to Drain. With parallel execution, the efficiency of Spell can be additionally improved by up to 4 times on the BGL dataset.


%\subsubsection{Memory footprint}\label{sec:mem}
%Nowadays, as log datasets in gigabytes have become commonplace, it is crucial for log parsers to sustain performance with large log files. However, compared to accuracy and efficiency, only a few works focused on evaluating the memory occupancy of existing log parsers. 
%For instance, as reported by Makanju et al.~\cite{makanju2011lightweight}, IPLoM, SLCT, and LogHound had around 6 times fewer virtual memory occupancies on small datasets. But on the relatively larger HPC dataset, LogHound suffered from memory crashes processing a file of 11.4~MB since the specified low support value leads to a massive number of item sets.
%Dai et al.~\cite{dai2020logram} reported that Spell crashed on datasets with 1G size due to its memory issues.
%Hamooni et al.~\cite{hamooni2016logmine} reported that LogMine has 16-61 times less memory occupancy than HALer on 5 datasets because the memory complexity of LogMine is only $O$(\#clusters) while HALer needs to compute the pairwise distances for all the input logs (i.e., $O(N)$ memory complexity).
%Zhang et al.~\cite{zhang2020efficient} measured the memory occupancy of Craftsman, IPLoM, LogSig, and LKE parsing the BGL dataset. Craftsman only required an average of 30.6 MB memory space thanks to its memory-efficient design, while LKE incurred up to 23.5 GB due to its large number of intermediate items.
%
%For example, as detailed in \cite{makanju2011lightweight}, Teiresias could not even process datasets larger than 9600 log messages and LogHound crashed when tested on the HPC dataset with long messages (up to 95) and a low number of target clusters (i.e., file support threshold equals to 2).
%LKE fails to parse large datasets in reasonable time~\cite{he2016evaluation,he2017drain,du2018spell}.
%Drain was observed to crash parsing log files with more than 300 k messages~\cite{messaoudi2018search}.


\subsection{Qualitative features}\label{sec:features}
There are several noteworthy operational features, including the parsing mode, preprocessing, and parameter tuning.
These features can help users understand the accessibility and suitability of each existing solution. We devote this section to discussing these qualitative features.  

\subsubsection{Parsing mode}
Existing log parsers can operate in three different modes, namely {\it online}, {\it offline}, and {\it hybrid}.
Offline log parsers need to process all the log messages in batches. 
Most of the relatively early log parsers such as SLCT, LKE, LogMine, and IPLoM operate offline.
Intuitively, offline parsing mode should lead to superior performance as it allows parsers to walk through all the messages and parse the logs globally. For instance, SLCT requires multiple passes on the input log messages to mine the frequent token sequences and extract the correct log templates.
However, offline parsers cannot allow for real-time log analytics, making them ill-suited for hyper-scale distributed systems. 

To cope with this challenge, many recent log parsers embrace the online streaming mode.
In fact, with the emergence of more specialized heuristics, online log parsers have managed to attain comparable (if not better) performance than their offline counterparts~\cite{he2017drain,du2018spell,dai2020logram}.
Online parsers such as Spell, Drain, and SHISO operate in a streaming fashion and can be readily integrated with log mining tools for data-driven analysis in real-time. They have two significant advantages over offline solutions. First off, online parsers can interpret newly collected logs on the fly and incrementally refine their internal parsing results without going through the offline training phase, making them ideal for real-time tasks such as system monitoring and fault diagnosis.
Offline log parsers generally fall short in this regard. Some solutions, such as LKE and LogSig, can even take days to parse large datasets.
Secondly, unlike offline solutions, online parsers do not need to load the entire input data (which can be prohibitively huge) into the memory space. This makes online parsers more accessible to users that do not possess enough resources. 

Besides these two standard modes, some log parsers operate in the hybrid mode, which entails an offline training phase and an online parsing phase, just like a typical machine learning pipeline. For instance, NuLog requires offline training to populate the model parameters via backward propagation. After that, it serves the model and parses the input logs in online mode. This self-supervised approach can better learn the characteristics of logs from different sources and overcome the limitations of heuristic approaches that fail to generalize for unobserved log formats.
According to our benchmarking results, NuLog renders the highest overall parsing accuracy. Such advantages have also been observed by other hybrid-mode log parsers~\cite{coustie2020meting,xiao2020lpv,nguyen2021logdtl}. Although more extensive experimental evaluations are still needed to prove the validity of these solutions, hybrid mode presents an intriguing direction for developers.

\subsubsection{Parameter tuning}\label{sec:tuning}
Most of the existing log parsers expose some parameters to allow users to fine-tune performance. Nonetheless, correctly tuning these parameters is a non-trivial task due to three reasons. First off, the exposed parameters usually have distinct sensitivities depending on the input data, which can only be understood through extensive benchmarking. For example, SLCT and LogCluster feature a support threshold used to locate frequent words from input logs. An overly strict threshold cannot identify all the relevant tokens and their associated patterns, while too loose thresholds further the computation overhead and may cause overfitting~\cite{vaarandi2015logcluster}. Second, the tunable parameters may have an implicit impact on each other, which requires a joint evaluation campaign to find the most suitable combination of parameters. Third, the tuning step must repeat for new logs to ensure the most desirable parsing results~\cite{zhu2019tools}. 
\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/tuning}
\caption{The general impact of parameter tuning.}
\label{fig:tuning}
\end{center}
\end{figure}

In this paper, we investigate the impact of parameter tuning. Based on the default parameters of each log parser, we sensibly change the values and collect the resulting PA. The same procedure is repeated on all the same 2k labeled datasets in Sec.~\ref{sec:accuracy}. To reflect this impact in a general sense, we calculate the ratio of optimal PA over the average PA, as shown in Fig.~\ref{fig:tuning}. 
According to our study, more tunable parameters do not necessarily mean higher tuning overhead. Some log parsers are relatively easy to tune because their parameters have negligible sensitivity. 
For instance, LogMine exposes two tunable parameters for its clustering phase, i.e., the maximal initial distance ($MaxDist_0$) and increasing factor ($\alpha$), representing a tradeoff between the accuracy and parsing time of log parsing. But the impact of these two parameters on the final result is very minimal. 
Similarly, SHISO has 4 parameters, i.e., the maximal child nodes and 3 format thresholds, that have little impact on the parsing accuracy.
IPLoM has 5 tunable parameters including file support thresholds, partition support threshold, cluster goodness threshold, and lower/upper bound. Based on our analysis, these parameters have relatively small influence and the file support threshold is the dominant parameter.  

On the other hand, some log parsers only expose a few parameters, but they require more careful tuning. 
For instance, 
Spell's message type threshold can hugely impact the parsing results (nearly $40\%$). Its split and merge thresholds are also tunable though less impactful.
LogSig has 2 tunable parameters, i.e., the number of event types ($k$) and the word pair step ($\lambda'$), that can cause $30\%$ difference. 
LKE exposes 3 tunable parameters: the edit distance weight, the cluster threshold, and the private contents threshold. These parameters need to be carefully set to avoid potential caveats. In particular, the authors of LKE even employed a K-Means algorithm to decide the cluster threshold. According to our experience, NuLog has the highest parameter tuning overhead. It exposes three parameters, i.e., \#epochs, $k$, \#samples, that can cover a vast range of values. The \#epoch has to be carefully tuned across different datasets and $k$ can only be fixed via cross-validation. We failed to attain even $20\%$ PA on the Linux dataset. 
In general, these solutions require deep understanding of their design internals and the characteristics of the input logs, which can be extremely challenging for other users. 
One way to reduce this overhead is to tune parameters on small samples and directly apply them on larger datasets. Although this transferred parameter tuning works decently in some scenarios, many solutions still fail to sustain satisfactory performance on large log files with more diverse message formats and event types, as detailed by He et al.~\cite{he2016evaluation}. 

%Some solutions expose even more parameters and thus incur even higher tuning overhead. 
%MoLFI has four parameters for its evolutionary algorithm, i.e., crossover probability, mutation probability, population size, and stopping condition. As the potential performance gain cannot compensate for the overhead of tuning these parameters, the authors opted to use the default values suggested by the related literature~\cite{messaoudi2018search}.
%POP also contains 4 parameters that need to be adjusted based on the datasets.


%Similarly, solutions like SHISO, POP, CAPRI, and IPLoM expose more than four tunable parameters and require an extensive sequence of microbenchmarks conducted on different values to pinpoint the most suitable set of parameters (e.g., through grid search~\cite{wang2021ltmatch}). A deep understanding of the algorithmic internals of each log parser and the characteristics of the input log files is also needed to accelerate the process and avoid potential caveats.

%There has been a research trend to automate this process to avoid the parameter tuning overhead and make log parsers more accessible to ordinary users. In particular,

Note that some solutions are designed with this difficulty in mind and thus do not require manual parameter tuning. For example, 
 Some open-source solutions, e.g., LFA, SwissLog, and Paddy, already avoids this step. Furthermore, 
Slop~\cite{zhao2018slop} defines a non-linear threshold criterion that can adapt to several system logs and thus does not require any manual parameter tuning. LogSimilarity~\cite{kimura2018proactive} employed an online classification algorithm to adjust the involved parameters incrementally.
Although existing research on automatic parameter tuning is still limited, it is a promising direction to implement new solutions that can be adaptive to different settings without human intervention.

\begin{figure}[!tb]
\begin{center}
\includegraphics[width=0.5\textwidth]{figures/preprocessing}
\caption{The average accuracy gain with preprocessing}
\label{fig:preprocessing}
\end{center}
\end{figure}

\subsubsection{Preprocessing}\label{sec:prep}
Besides parameter tuning, existing solutions also heavily rely on human involvement for preprocessing, which may consist of interpreting raw log messages, removing irrelevant tokens, and substitute redundant tokens (such as timestamps, IP addresses, unique identifiers) to reduce the parsing noise and enhance the overall performance. 
All the open-source solution we have evaluated rely on empirically composed regular expressions for preprocessing. 
According to prior research, log parsers can generally benefit from fine-grained preprocessing based on the characteristic of the input logs. But this has to be conducted with caution, as incorrect preprocessing may inversely lead to performance degradation~\cite{liu2020fastlogsim,he2016evaluation,he2017towards}. It is thus necessary to understand the impact of preprocessing on existing log parsers. 

In this part, we rerun the accuracy tests without the preprocessing step on all the 2k datasets and compare the difference with the corresponding original accuracy. The average ratio of original PA over the non-preprocessing PA for each solution is illustrated in Fig.~\ref{fig:preprocessing}. According to our test results, preprocessing has little impact on LFA, Drain, SwissLog, and AEL, which makes them relatively accessible to users without prior knowledge of the input logs. On the contrary, the accuracies of Lenma and LogCluster highly depend on the preprocessing. In particular, on the Proxifier dataset, they can only achieve $0.1\%$ PA without preprocessing. SHISO, SLCT, and LogSig also presents huge difference on some datasets. These solutions require more specialized preprocessing rules to unleash their full potential. 
%Drain, Logram, FastLogSim, NuLog, CLF, and LKE allow users to empirically compose regular expressions to filter out redundant tokens from the raw log data. In particular, FastLogSim specifies a set of regular expressions to replace irrelevant variables (e.g., IPs, URLs, file paths, and application names) with predefined tokens.
%In addition to regular expressions, some solutions also employ specialized rules for preprocessing. 
%For instance, 
%Stearley et al.~\cite{stearley2004towards} required to map each input word token into a unique integer and strings containing the equal signs split into two tokens. It also omits several irrelevant message fields, including timestamps, message sources, and process IDs.
%AEL heavily relies on user-specified filtering rules to identify various parts of the log messages.
%SLCT and LogCluster enable several command-line options for users to specify preprocessing rules based on prior knowledge of the target dataset.
%Delog further defines rules to remove redundant logs and reduce the computation overhead to enable automatic preprocessing.

Although regular expressions are widely used by existing solutions, they are still too general and do not provide customized preprocessing for individual parsers. In some rare cases, we have even observed sightly decreased accuracy due to preprocessing in our previous tests. 
To this end, some log parsers feature more advanced preprocessing procedures using domain-specific knowledge.
For example, POP provides two types of preprocessing functions for users to trim redundant fields and prioritize specific log events.
Pylogabstract integrates nerlogparser~\cite{studiawan2018automatic} to perf  orm automatic preprocessing through named entity recognition.
%LogMine encompasses tokenization and type detection methods in its preprocessing phase to improve parsing accuracy.
%In LogSig, users can decide the required signature number based on their domain knowledge. It also allows users to specify a set of domain-specific features (such as regular expressions) and message signature constraints.
Aside from the empirical understanding of input data, some solutions can benefit from detailed knowledge of the target systems.
For instance, LogTree relies on grammar parsers to preprocess log data and build the hierarchical message segments. These grammar parsers are highly dependent on specific system programs and usually require prior knowledge of the relevant domains. Users can also specify different clustering algorithms based on their needs, e.g., LEARNPADS~\cite{zhu2010incremental} requires a user-specified log format description to preprocess log entries. 
Although these solutions enable more sophisticated parsing by consolidating user experiences and domain-specific knowledge, they are also more difficult for average users to handle.

Another critical aspect of preprocessing, as pointed out by existing works, is how to handle the delimiters for heterogeneous logs. Most existing solutions, such as Spell, consider the commonly used signs such as space and equal as delimiters. Nonetheless, such an assumption does not always hold due to the free-text nature of system log messages, which can result in unexpected parsing errors~\cite{makanju2011lightweight}. Some solutions try to tackle this issue by simultaneously considering multiple signs as delimiters~\cite{li2020swisslog,wurzenberger2019aecid,tovarvnak2019normalization}. For instance, SwissLog employs a set of 5 delimiters (\{, . ; : "\}) to tokenize the raw log messages more precisely. 
One-to-One allows users to specify the delimiters based on knowledge of the input log formats. 
Although these methods can alleviate the tokenization mistake, they cannot altogether avoid it since log entries can always employ more distinctive characters as delimiters.
To overcome this limitation, {Wurzenberger et al.~\cite{wurzenberger2020creating}} proposed a character-based log parser that performs a character-wise comparison to evaluate the similarity of two log messages, avoiding the entire tokenization step. Although their evaluation results were promising, this novel approach is still in its infancy, and more extensive benchmarking is needed to validate its applicability and performance comprehensively. 

\begin{table*}[!tb]
%\renewcommand{\arraystretch}{0.5}
\centering
\footnotesize
\caption{Qualitative features of some existing log parsing solutions. For each log parser, we list its parsing mode (i.e., offline, online, and hybrid), number of tunable parameters and the level of tuning complexity (i.e., high, medium, low, and none), preprocessing method, compatible delimiters (e.g., white-space (WS), punctuation marks), and code availability.}
\begin{tabular}{|l||ccc|cc|cc|c|}
\hline 
\multirow{2}{*}{\bf Log parsers}  & \multicolumn{3}{c|}{\bf Parsing mode} & \multicolumn{2}{c|}{\bf Parameter tuning}  & \multicolumn{2}{c|}{\bf Reliance on Preprocessing} &\bf Open \\ \cline{2-8}
& Offline & Online & Hybrid & Parameters & Complexity & Method & Delimiters &\bf  source \\ \hline \hline
\bf SLCT~\cite{vaarandi2003data} & \checkmark & & & 2 & Low & RegEx-based processing & User-specified & \checkmark \\\hline
%\bf LogHound~\cite{vaarandi2004breadth} & \checkmark & && 2 & Low & RegEx-based processing & User-specified & \checkmark \\ \hline
\bf LFA~\cite{nagappan2010abstracting} & \checkmark & & & - & - & - & - & \checkmark \\ \hline
%\bf ENG~\cite{tovarvnak2019normalization}  &&&&&&&& \\ \hline 
\bf LKE~\cite{fu2009execution} & \checkmark & & & 3 & Medium & RegEx-based processing & WS & \checkmark \\ \hline
%\bf LEARNPADS~\cite{zhu2010incremental} &  & \checkmark &&&&&& \\ \hline
\bf LogCluster \cite{vaarandi2015logcluster} & \checkmark &&& 3 & Medium & RegEx-based processing & User-specified & \checkmark \\ \hline
\bf LenMa~\cite{shima2016length} & & \checkmark && 1 & Low & Rule-based processing & - & \checkmark \\ \hline
\bf LogMine \cite{hamooni2016logmine} & \checkmark & & & 2 & Low & Tokenization, filtering & WS & \checkmark \\ \hline
\bf AEL~\cite{jiang2008abstracting,jiang2008automated} & \checkmark & & & - & - & Rule-based processing & WS & \checkmark \\ \hline
\bf LogSig~\cite{tang2011logsig}  & \checkmark & & & 2 & Medium & RegEx-based processing & - & \checkmark  \\ \hline
\bf MoLFI~\cite{messaoudi2018search} & \checkmark & & & 4 & Medium & RegEx-based processing & WS, puctuations  & \checkmark \\ \hline
%\bf POP~\cite{he2017towards}  & & \checkmark & & 4 & Medium & Function-based or RegEx & - &  \xmark \\ \hline
%\bf HLAer~\cite{ning20141hlaer} & & & \checkmark & 2 & Low & User-defined tokenization & User-specified & \xmark \\ \hline
%{\bf LTE~\cite{ya2015automatic}}  &&&&&&&& \\ \hline
%\bf LogTree~\cite{tang2010logtree} & \checkmark &&& 5 & High & Rule-based processing & WS : , `` "& \xmark \\ \hline
%\bf HELO~\cite{gainaru2011event} & & & \checkmark & 1 & Low & - & - & \xmark \\ \hline
\bf IPLoM~\cite{makanju2009clustering,makanju2011lightweight} & \checkmark & & & 6 & High & Tokenization & WS & \checkmark \\ \hline
%\bf CAPRI~\cite{zulkernine2013capri}  & \checkmark & & & 5 & High & Rule-based type cast & WS & \checkmark \\ \hline
\bf SHISO~\cite{mizutani2013incremental} & & \checkmark && 4 & Medium & Rule-based conversion & WS \# = &  \checkmark\\ \hline
\bf Drain~\cite{he2017drain} & & \checkmark & & 2 & Low & RegEx-based processing & - & \checkmark \\ \hline
\bf Spell~\cite{du2016spell,du2018spell} & & \checkmark & & 3 & Medium & RegEx-based processing & User-specified & \checkmark \\ \hline
%\bf Slop~\cite{zhao2018slop} & & \checkmark & & 0 & - & Word filtering & WS & \xmark \\ \hline
%\bf One-to-one~\cite{chunyong2020log} & & \checkmark & & - & - & Rule-based processing & User-specified & \xmark \\ \hline
%\bf CLF~\cite{zhang2019efficient} & \checkmark & & & - & - & RegEx-based processing  & - & \xmark \\ \hline
%\bf LogOHC~\cite{yang2019online} &  & \checkmark & & 6 & High & Vectorization algorithm & - & \xmark \\ \hline
%\bf Logan~\cite{agrawal2019logan} &  & \checkmark & & 0 & None & RegEx-based processing & WS & \xmark \\ \hline
\bf Logram~\cite{dai2020logram} & \checkmark & \checkmark &  & - & - & RegEx-based processing & WS & \checkmark \\ \hline
%\bf Delog~\cite{agrawal2019delog} & \checkmark & & & 3 & Medium & RegEx-based processing & WS & \xmark \\ \hline
%\bf FLP~\cite{zhong2018flp} & & \checkmark & & - & - & RegEx-based processing & - & \checkmark \\ \hline
\bf NuLog~\cite{nedelkoski2020self} & & & \checkmark & 2 & Medium &User-defined tokenization & User-specified  & \checkmark \\ \hline
%\bf AECID-PG~\cite{wurzenberger2019aecid} & & \checkmark && 9 & High & User-defined tokenization & User-specified & \checkmark \\ \hline
%\bf Pylogabstract~\cite{studiawan2020automatic}  & \checkmark & && 0 & None & Automatic & WS & \checkmark \\ \hline
\bf Paddy~\cite{huang2020paddy} & & \checkmark & & 2 & Low & RegEx-based processing & - & \checkmark \\ \hline
%\bf FastLogSim~\cite{liu2020fastlogsim} & \checkmark &&& 1 & Low & RegEx-based processing & - & \xmark \\ \hline
\bf SwissLog~\cite{li2020swisslog} & & & \checkmark & 0 & None & Dictionary-based matching & WS , . ; : '' & \checkmark \\ \hline
%\bf Baler~\cite{taerat2011baler} & \checkmark &&& 2 & Low & RegEx-based processing  & - & \xmark \\ \hline
%\bf Lopper~\cite{liu2019lopper}  & & \checkmark & & - &  - & RegEx-based processing & - & \xmark \\ \hline
%\bf METI$N$G~\cite{coustie2020meting} & & & \checkmark & 2 & Low & IP or Number replacement & - & \xmark \\ \hline
%\bf OLMPT~\cite{wen2020olmpt} & & \checkmark & & - & - & Word filtering, replacement & WS & \xmark \\ \hline
%\bf LPV~\cite{xiao2020lpv} & & & \checkmark & 6 & High & Word filtering, replacement & WS ( ) = [ ] : ? & \xmark \\ \hline
%\multirow{2}{*}{\bf FlexParser~\cite{ruecker2021flexparser}} & & & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{-} & \multirow{2}{*}{Medium} & Word filtering, conversion,  & \multirow{2}{*}{-}& \multirow{2}{*}{\xmark} \\ 
%&&&&& & tokenization, vectorization & & \\ \hline
%\bf LogDTL~\cite{nguyen2021logdtl} & & & \checkmark & - & Low & ML-based data preparation & - & \checkmark \\ \hline
%\bf LTmatch~\cite{wang2021ltmatch} & & \checkmark &  & 3 & Medium & IP or Number replacement & - & \xmark \\ \hline
%\bf Prefix-Graph~\cite{chu2021prefix} & &  & \checkmark & 1 & Low & Number replacement & - & \xmark \\ \hline
%\bf template2Vec~\cite{meng2019loganomaly} &&&&&&&& \\ \hline
%\bf Log2vec~\cite{meng2020semantic} &&&&&&&& \checkmark \\ \hline
%\bf OILog~\cite{duan2021oilog} &&&&&&&& \xmark \\ \hline
%\bf FT-tree~\cite{zhang2017syslog} &&&&&&&& \\ \hline 
%&&&&&&&& \\ \hline
\end{tabular}
\label{tab:feature}
\end{table*}





